System Performance with varying L1 Instruction and Data Cache Sizes: An Empirical Analysis

In this project, we investigate the fluctuations in performance caused by changing the Instruction (I-cache) size and the Data (D-cache) size in the L1 cache. We employ the Gem5 framework to simulate a system with varying specifications on a single host machine. We utilize the FreqMine benchmark available under the PARSEC suite as the workload program to benchmark our simulated system. The Out-order CPU (O3) with Ruby memory model was simulated in a Full-System X86 environment with Linux OS. The chosen metrics deal with Hit Rate, Misses, Memory Latency, Instruction Rate, and Bus Traffic within the system. Performance observed by varying L1 size within a certain range of values was used to compute Confidence Interval based statistics for relevant metrics. Our expectations, corresponding experimental observations, and discrepancies are also discussed in this report.

==> notes.tex <==
Phase 3. Final Report (45 points; due Tuesday November 19)

This final report should present the graphs illustrating the results and their interpretation. The submission includes the following sections:

a.  The contents of OptionSelection and ExperimentDesign from Phases 1 and 2, respectively.

b.  What changes relative to the original experiment profile and experiment design were made, and why.

c.  The statistical processing of the results. It is desirable to include, confidence intervals for the results. This is only possible if individual runs take no more tha say 30 minutes. In this case you need to carry out each run multiple times, e.g., 10 times, compute the average of the result and repeat this process several times, say 8-10 times then use the statitics to compute 95\%  85\% confidence intervals (CIs). You can use an online CI calculator at https://www.mathsisfun.com/data/confidence-interval-calculator.html 

d.  Individual plots of the results including an in-depth discussion of each plot. See also the exaple projects folder.

e.  Discussion of abnormalities, unexpected behavior.

f. Comparation with what you expected.

g.  Comparison with similar results in the literature if any.

h.  What are the main things that you learned from this project.

D. Grading Only projects choosing options: 2b, 3c or 3d, and 7a can get a maximum score of 100 points. Projects choosing any of the following options 2a, 3a, or 3b could only get a maximum score of 85 points. Extra points for using: option 1 (+5), option 4b (+6), confidence intervals (+10).






\section{Option Seclection}


\section{Related Work}



\section{Experiment Design}



\section{Experimental Results}

%What changes relative to the original experiment profile and experiment design were made, and why.


\section{Qualitative Analysis}

%Individual plots of the results including an in-depth discussion of each plot. See also the exaple projects folder.
%Table of all results for all sim sizes

\section{Statistical Analysis}

%The statistical processing of the results. It is desirable to include, confidence intervals for the results. This is only possible if individual runs take no more tha say 30 minutes. In this case you need to carry out each run multiple times, e.g., 10 times, compute the average of the result and repeat this process several times, say 8-10 times then use the statitics to compute 95\%  85\% confidence intervals (CIs). You can use an online CI calculator at https://www.mathsisfun.com/data/confidence-interval-calculator.html 


\section{Conclusion}


\section{Discussion}
%Discussion of abnormalities, unexpected behavior.
%Comparation with what you expected.
%Comparison with similar results in the literature if any.
%What are the main things that you learned from this project.




% During submission Leave comment on Extra points for using: option 1 (+5), option 4b (+6), confidence intervals (+10)
